Mid-to-Far Infrared Spectral Energy Distribution of Galaxies in Spitzer First Look Survey Field

We made model fitting to the mid-to-far infrared spectral energy distributions (SEDs) for different categories of galaxies in the main extragalactic field of the {\it Spitzer} First Look Survey with the aid of spectroscopic information from the Sloan Digital Sky Survey. We find that the mid-to-far infrared SEDs of HII galaxies, mixture type galaxies and LINERs can be well fitted by the one-parameter ($\alpha$) dust model of Dale et al. plus the 13 Gyr dust-free elliptical galaxy model. The statistics of $\alpha$ values indicates that all these galaxies tend to be quiescent, although the HII galaxies are relatively more active than the LINERs. The mid-infrared SEDs of absorption galaxies are well fitted simply by the 13 Gyr dust-free elliptical galaxy template, and the near-to-mid infrared SEDs of QSOs can be represented by AGN NGC 5506.

==> readme <==
Title:   Mid-to-Far Infrared Spectral Energy Distribution of Galaxies in Spitzer First Look Survey Field
Authors:   Xiao-Qing Wen (1,2), Hong Wu (2), Chen Cao (2), and Xiao-Yang Xia (1,2) 
    ((1)Department of Physics, Tianjin Normal University (2) National Astronomical Observatories, Chinese Academy of Sciences) 

We made model fitting to the mid-to-far infrared spectral energy distributions (SEDs) for different categories of galaxies in the main extragalactic field of the {\it Spitzer} First Look Survey  with the aid of spectroscopic information from the Sloan Digital Sky Survey. We find that the mid-to-far infrared SEDs of HII galaxies, mixture type galaxies and LINERs can be well fitted by the one-parameter ($\alpha$) dust model of Dale et al.  plus the 13 Gyr dust-free elliptical galaxy model. The statistics of $\alpha$ values indicates that all these galaxies tend to be quiescent, although the HII galaxies are relatively more active than the LINERs. The mid-infrared SEDs of absorption galaxies are well fitted simply by the 13 Gyr dust-free elliptical galaxy template, and the near-to-mid infrared  SEDs of QSOs can be represented by AGN NGC~5506.

Comments:  12 pages with 8 figures, will be appeared in ChJAA, Vol.7 (2007), No.2  

